Apple Intelligence Foundation Language Models

We present foundation language models developed to power Apple Intelligence features, including a ~3 billion parameter model designed to run efficiently on devices and a large server-based language model designed for Private Cloud Compute. These models are designed to perform a wide range of tasks efficiently, accurately, and responsibly. This report describes the model architecture, the data used to train the model, the training process, how the models are optimized for inference, and the evaluation results. We highlight our focus on Responsible AI and how the principles are applied throughout the model development.

==> tables/human_eval_main.tex <==
\begin{table}[!ht]
    \color{red} %
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{@{}lrrr|lrrr@{}}
            \toprule
                       & \multicolumn{3}{c}{\ourmodel{-on-device}} &              & \multicolumn{3}{c}{\ourmodel{-server}}   \\
            \cmidrule(lr){2-4} \cmidrule(lr){6-8}  
            model         & win                                & tie    & loss    &                            model          & win    & tie    & loss  \\
            \midrule

            Gemma-2B   & 63.8\% & 21.0\% & 15.2\%   & DBRX-Instruct         & 56.4\% & 24.6\%  & 19.0\%   \\
            \mistral{} & 50.7\% & 24.7\% & 24.6\%   & GPT-3.5               & 51.5\% & 27.4\%  & 21.1\%  \\
            \phimini{} & 47.7\% & 24.2\% & 28.1\%   & Mixtral 8x22          & 44.9\% & 29.3\%  & 25.8\%  \\
            Gemma-7B   & 43.7\% & 26.8\% & 29.5\%   & Llama 3 70B           & 31.7\% & 33.0\%  & 35.3\% \\  
            Llama 3 8B & 29.7\% & 32.0\% & 38.3\%   & GPT-4                 & 29.3\% & 31.9\%  & 38.8\%   \\
            \bottomrule
        \end{tabular}
    }
    \caption{Data for \autoref{fig:human-eval}.}
    \label{tab:human_eval_main}
\end{table}




==> tables/human_eval_safety.tex <==

\begin{table}[!ht]
    \color{red} %
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{@{}lr|lr@{}}
        \toprule
      Model & Violation Rate (\%) & Model & Violation Rate (\%)  \\
      \midrule
         \ourmodel{-on-device} & 7.5 & \ourmodel{-server} & 6.3  \\
        \midrule
        \gemmas & 13.9   & DBRX-Instruct  &  43.7  \\
        \mistral &    51.3     & \gpts  & 22.6 \\
        \phimini{} &  24.4    & Mixtral 8x22B  & 47.5 \\
         \gemmal &  13.6     & \gptl & 28.8 \\
         Llama 3 8B &  21.8  & Llama 3 70B & 27.9\\
   \bottomrule
    \end{tabular}
    }
    \caption{Data for \autoref{fig:human-eval-harmfulness}}
    \label{tab:human_eval_single_side_safety}
\end{table}

\begin{table}[!ht]
    \color{red} %
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{@{}lrrr|lrrr@{}}
        \toprule
        & \multicolumn{3}{c}{\ourmodel{-on-device}} & & \multicolumn{3}{c}{\ourmodel{-server}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){6-8}
        model & win & tie & loss & model & win & tie & loss \\ 
        \midrule
         \gemmas & 54.0 & 33.3 & 12.7 & Mixtral 8x22B & 67.0 & 25.1 & 7.9 \\
         \phimini{} & 61.2 & 29.0 & 9.8   & \gpts & 59.4 & 29.2 & 11.4 \\
         \mistral & 70.6 & 23.2 & 6.2 & DBRX-Instruct & 66.8 & 24.5 & 8.7 \\ 
        \gemmal & 42.9 & 41.5  & 15.6 & \gptl & 62.2 & 28.7 & 9.1 \\
         Llama 3 8B & 60.4 & 30.0 & 9.6 &  Llama 3 70B &  64.4 & 28.6 & 7.0\\
        \bottomrule
    \end{tabular}
    }
    \caption{Data for \autoref{fig:human-eval-sxs}}
    \label{tab:human_eval_sxs_safety}
\end{table}































==> tables/if_eval.tex <==




\begin{table}[!ht]
    \color{red} %
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}lrrrrrr@{}}
            \toprule
                                       & \ourmodel{-on-device} & Gemma-2B & Phi-3-mini & Gemma-7B & Mistral-7B & Llama 3-8B \\
            \midrule
            IFEval Instruction-level & \bftab 85.7       & 40.5     & 67.9       & 61.6     & 65.2  & 82.5 \\
            IFEval Prompt-level      & \bftab 79.3       & 28.7     & 57.8       & 51.4     & 54.2  & 74.7 \\
            AlpacaEval 2.0 LC        & 23.6       & 13.9     & 20.5       & \bftab 29.5     & 17.1  & 22.9\\
            \bottomrule
        \end{tabular}
    }
    \caption{Data for \autoref{fig:instruction-following}}
    \label{tab:if_eval_only_on_device}
\end{table}


\begin{table}[!ht]
    \color{red} %
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}lrrrrrr@{}}
            \toprule
                                        &  \ourmodel{-server} & GPT-3.5 & Llama 3-70B & GPT-4   & \dbrx{} & Mixtral-8$\times$22B \\
            \midrule
            IFEval Instruction-level &   \bftab 88.5    & 74.8     &  88.1    & 85.4   & 65.8  & 79.4   \\
            IFEval Prompt-level      &   \bftab 83.0    & 65.3     &  82.3    & 79.3   & 53.6  & 71.4   \\
            AlpacaEval 2.0 LC        &       47.1    & 22.7     & 34.4    & \bftab 54.6   & 25.4  & 30.9   \\
            Arena Hard        &       35.5    & 23.3     & 46.6    &  \bftab 78.0   & 23.9  & 36.4   \\
            \bottomrule
        \end{tabular}
    }
    \caption{Data for \autoref{fig:instruction-following}}
    \label{tab:if_eval_only_server}
\end{table}





==> tables/math_eval.tex <==
\begin{table}[!ht]
    \color{red} %
    \centering
    \begin{tabular}{@{}lrr@{}}
        \toprule
        \textbf{Model} & \textbf{GSM8K (8-shot)} & \textbf{MATH (4-shot)} \\
        \midrule
        Gemma-7B & 49.9 & 17.3 \\
        \mistral{}            & 41.7   & 11.5    \\
        \ourmodel{-on-device}        & 64.0  & \bftab 26.1    \\
        Llama 3 8B & 75.8 & 24.3 \\
        \phimini{}  & \bftab 78.5 & 21.8 \\
        \midrule
        GPT-3.5                & 76.3   & 33.9    \\
        Mixtral-8x22B          & 77.8   & 41.1    \\
        \ourmodel{-server}        & 83.3  & 42.3    \\
        Llama 3 70B & 86.8 & 41.7 \\
        GPT-4                & \bftab 88.6   & \bftab 43.6    \\
        \bottomrule
    \end{tabular}
    \caption{Data for \autoref{fig:math}}
    \label{tab:math_eval}
\end{table}


==> tables/summarization_domain.tex <==




        

        

\begin{table}[t]
    \color{red} %
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lrrrrrr@{}}
        \toprule
        \textbf{Model}  & \multicolumn{3}{c}{\textbf{Good Result Ratio}}  & \multicolumn{3}{c}{\textbf{Poor Result Ratio}} \\
                        & Email & Message & Notification & Email & Message & Notification \\
        \midrule
        \ourmodel-on-device-adapter{}  & \bftab 71.3\% & \bftab 63.0\% & \bftab 74.9\%   & 7.2\% & \bftab 15.9\% & \bftab 10.0\% \\
        \phimini{} & 44.7\% & 32.8\% & 56.6\% &   12\% & 31.4\% & 18.3\%\\
        \llamathrees{} & 36.1\% & 21.3\% & 27.7\%   & 12.8\% & 35.3\% & 48.3\%\\
        \gemmal{}  &  70.9\%  & 51.1\% & 60.9\%   & \bftab 4.5\% & 18.3\% & 12.9\%\\
        \bottomrule
    \end{tabular}
    }
    \caption{Data for \autoref{fig:summ-human-eval}}
    \label{tab:sum_prod_human_eval3}
\end{table}


        


==> tables/tool_use_eval.tex <==
\begin{table}[!ht]
    \color{red} %
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lrrrrrr@{}}
        \toprule
        \textbf{Model}  & \multicolumn{6}{c}{\textbf{Gorilla}} \\
                        & Simple & Multiple & Parallel & Parallel Multiple & Relevance & Average \\
        \midrule
        \ourmodel{-on-device}  & 89.0 & 90.0 & 76.0 & 65.0 & 81.0 & 80.2 \\
        \ourmodel{-server} & 91.0 & 95.5 & 84.5 & 85.0 & 91.3 & \bftab 89.5 \\
        \midrule
        \gemininext{-0514} & 80.2 & 92.0 & 91.5 & 88 & 89.6 & 88.3 \\
        GPT-3.5 & 61.5 & 66.0 & 91.0 & 81.0 & 2.1 & 60.3 \\
        GPT-4 & 80.2 & 93.0 & 90.5 & 84.5 & 82.9 & 86.2 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Data for \autoref{fig:tool-use}} \label{tab:tool_use_eval}
\end{table}



==> tables/writing_eval.tex <==
\begin{table}[!ht]
    \color{red} %
    \centering
    \begin{tabular}{@{}lrrrr@{}}
        \toprule
        \textbf{Model}  & \multicolumn{1}{c}{\textbf{Summarization}} & \multicolumn{1}{c}{\textbf{Composition}}    \\
        \midrule
        \phimini{}      & 8.8                                        & 9.0                                      \\
        \gemmas{}       & 7.6                                        & 8.0                                      \\
        \gemmal{}       & 8.9                                        & \bftab 9.1                             \\
        \mistral{}      & 8.9                                        & \bftab 9.1                             \\
        \ourmodel{-on-device}  & \bftab 9.1                               & 9.0                             \\
        \midrule
        GPT-3.5          & 8.6                                        & 8.9                                      \\
        \dbrx{}         & 9.2                                        & 9.2                                      \\
        \mixtrall{}     & \bftab 9.5                                    & 9.5                                      \\
        \ourmodel{-server} & \bftab 9.5                                    & 9.6                                      \\
        GPT-4            & \bftab 9.5                               & \bftab 9.7                             \\
        \bottomrule
    \end{tabular}
    \caption{Data for \autoref{fig:writing}}
    \label{tab:writing_eval}
\end{table}

